Selectively Informative Description can Reduce Undesired Embedding Entanglements in Text-to-Image Personalization

In text-to-image personalization, a timely and crucial challenge is the tendency of generated images overfitting to the biases present in the reference images. We initiate our study with a comprehensive categorization of the biases into background, nearby-object, tied-object, substance (in style re-contextualization), and pose biases. These biases manifest in the generated images due to their entanglement into the subject embedding. This undesired embedding entanglement not only results in the reflection of biases from the reference images into the generated images but also notably diminishes the alignment of the generated images with the given generation prompt. To address this challenge, we propose SID~(Selectively Informative Description), a text description strategy that deviates from the prevalent approach of only characterizing the subject's class identification. SID is generated utilizing multimodal GPT-4 and can be seamlessly integrated into optimization-based models. We present comprehensive experimental results along with analyses of cross-attention maps, subject-alignment, non-subject-disentanglement, and text-alignment.

==> Suppl_TEX/40.old_Failure_Cases_GPT-4.tex <==
\section{Failure cases with GPT-4}
\label{sec: Supple_failure cases with GPT-4}
\input{Suppl_TEX/941.Failure_cases}
While GPT-4~\cite{openai2023gpt4} generally generates descriptions that closely match the provided instructions, occasional failures do occur. In \cref{fig:failure cases of GPT-4}, we report two instances where GPT-4 does not generate prompts that align closely with the properties of SID.

==> Suppl_TEX/936_1.Multi_vs_DB_biased.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_biased/Multi_vs_DB_1_1.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_biased/Multi_vs_DB_1_2.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_biased/Multi_vs_DB_1_3.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_biased/Multi_vs_DB_1_5.png}
    \vspace{0.2cm}

    \caption{biased examples}
    % \label{fig:vs_Neg_Seg}
\end{figure*}

==> Suppl_TEX/937_1.Multi_vs_DB_diverse_but.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_but/Multi_vs_DB_2_1.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_but/Multi_vs_DB_2_2.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_but/Multi_vs_DB_2_3.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_but/Multi_vs_DB_2_4.png}
    \vspace{0.2cm}

    \caption{diverse but entangled, 1st (backgound mountain), 2nd (rocky surface), 3rd (nearby teapot, saurcer, filled in flower), last ( grassy field)}
    % \label{fig:vs_Neg_Seg}
\end{figure*}

==> Suppl_TEX/938_1.Multi_vs_DB_diverse_not.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_not/Multi_vs_DB_3_1.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_not/Multi_vs_DB_3_2.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_not/Multi_vs_DB_3_3.png}
    \vspace{0.2cm}

    \includegraphics[width=0.9\textwidth]{Figures/Appendix/Multi_vs_DB_diverse_not/Multi_vs_DB_3_4.png}
    \vspace{0.2cm}

    \caption{biased examples}
    % \label{fig:vs_Neg_Seg}
\end{figure*}

==> Suppl_TEX/X0.Quantitative_analysis_Fig2.tex <==
\section{Quantitative comparison between the description cases.}
To perform quantitative comparison on ~~~.
9개의 subject, 각 subject 당 4~6장 이미지, subject에 속하는 이미지가 거의 비슷한 content를 공유하는 bias가 심한 이미지로 선별
이렇게한 이유는 bias가 심한 challenging한 상황을 고려하기 위해, 여러 이미지에 대해 하나의 training description만 사용해서 분석의 편의성을 높이기 위해.
% \input{Suppl_TEX/01.Table_Quantitative_Fig2}

% use 9 subject, each subject consist of 4~6 reference images, and 


==> Suppl_TEX/X0.Random_Multi.tex <==
...


\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{Figures/overall.png}
\vspace{0.2cm}

\includegraphics[width=0.9\textwidth]{Figures/overall.png}
\vspace{0.2cm}

\includegraphics[width=0.9\textwidth]{Figures/overall.png}
\vspace{0.2cm}

\includegraphics[width=0.9\textwidth]{Figures/overall.png}
\caption{hello}
\label{fig:prompt_ablation_blueberry_bowl}
\end{figure*}



==> TEX/1010.Figure_facial.tex <==
\begin{figure}[t]
    \centering
\includegraphics[width=\columnwidth]{Figures/Limitation/facial_expression.png}
\vspace{-0.5cm}
    \caption{\textbf{Limitation in disentangling strong facial expressions.} Even when SID is applied, SID-integrated models struggle with disentangling strong facial expressions.}
    % \caption{\textbf{Failure cases in disentangling specific facial expressions.} Our approach struggles with expressions like \emph{tongue out} in contrast to the successful handling of a \emph{plain} dog facial expression in \cref{fig:main_bias} (last row).}    
    \vspace{-0.5cm}
    \label{fig:facial_expression}
\end{figure}


==> TEX/name.tex <==
% \newcommand{\rulesep}{\unskip\ \vrule\ }


\begin{figure*}[t!]
\centering
\renewcommand\twocolumn[1][]{#1}%
\hspace{1cm}
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny Train samples
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.45\textwidth}{%
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}}
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/01.jpg}}
    }
    \hspace{-0.14cm}
    \parbox{.45\textwidth}{%
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/00.jpg}}
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/04.jpg}}  
    }
}
\caption*{\centering\scriptsize bowl}
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.45\textwidth}{%
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/purse_perufme/00.jpg}}
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/purse_perufme/01.jpg}}
    }
    \hspace{-0.14cm}
    \parbox{.45\textwidth}{%
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/purse_perufme/02.jpg}}
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/purse_perufme/03.jpg}}  
    }
}
\caption*{\centering\scriptsize perfume}
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.45\textwidth}{%
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/blouse_skirt/00.jpg}}
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/blouse_skirt/01.jpg}}
    }
    \hspace{-0.14cm}
    \parbox{.45\textwidth}{%
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/blouse_skirt/02.jpg}}
        \frame{\includegraphics[width=\hsize]{Figures/Train_samples/blouse_skirt/03.jpg}}  
    }
}
\caption*{\centering\scriptsize blouse}
\end{subfigure}
\rulesep
% \hspace{0.05cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (a) Baseline
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\hspace{-0.2cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (b) Descriptive
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\hspace{-0.2cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (c) Details
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\hspace{-0.2cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (d) List
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\hspace{-0.2cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (e) Wrong relation
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\hspace{-0.2cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (f) Bias 1
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\hspace{-0.2cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (g) Bias 2
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\hspace{-0.2cm}
% 
% 
\begin{subfigure}[c]{0.10\textwidth}
\centering
\tiny (h) Wrong object
\vskip1em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\vskip0.5em
\parbox{\textwidth}{
    \centering
    \parbox{.92\textwidth}{%
        \includegraphics[width=\hsize]{Figures/Train_samples/berry_bowl/02.jpg}
    }
}
\caption*{\centering\scriptsize  }
\end{subfigure}
\end{figure*}




==> Table/Negative_Prompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method            & \begin{tabular}[c]{@{}c@{}}Text\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Image\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Subject\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Background\\ Alignment\end{tabular} \\
\midrule
Dreambooth        & 0.290                                                    & \textbf{0.781}                                            & 0.686                                                       & 0.701                                                          \\
Dreambooth + Neg. & 0.303                                                    & 0.722                                                     & 0.678                                                       & 0.655                                                          \\
Dreambooth + Seg. & 0.305                                                    & 0.716                                                     & \textbf{0.704}                                              & \textbf{0.650}                                                 \\
Dreambooth + Ours & \textbf{0.317}                                           & 0.718                                                     & 0.681                                                       & 0.651                                                         \\
\bottomrule
\end{tabular}%
}
\caption{Other disentanglement methods.}
\label{tab:neg_seg}
\end{table}

==> Table/One_shot.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccccccc}
\toprule
Method                            & Training prompt & CLIP-T         & CLIP-I         & DINO-I         & \begin{tabular}[c]{@{}c@{}}Subject\\ CLIP-I\end{tabular} & \begin{tabular}[c]{@{}c@{}}Subject\\ DINO-I\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bias \\ CLIP-I\end{tabular} & \begin{tabular}[c]{@{}c@{}}Bias \\ DINO-I\end{tabular} \\
\midrule
\multirow{2}{*}{Dreambooth}       & Baseline        & 0.301          & \textbf{0.788} & \textbf{0.603} & 0.705                                                    & \textbf{0.457}                                           & 0.721                                                  & 0.377                                                  \\
                                  & Ours            & \textbf{0.311} & 0.764          & 0.572          & \textbf{0.715}                                           & 0.452                                                    & \textbf{0.676}                                         & \textbf{0.307}                                         \\
\midrule
\multirow{2}{*}{Custom Diffusion} & Baseline        & 0.281          & \textbf{0.814} & \textbf{0.654} & 0.723                                                    & \textbf{0.501}                                           & 0.756                                                  & 0.436                                                  \\
                                  & Ours            & \textbf{0.309} & 0.773          & 0.587          & \textbf{0.723}                                           & 0.465                                                    & \textbf{0.690}                                         & \textbf{0.327}                                        \\
\midrule
\end{tabular}%
}
\caption{One shot}
\label{tab:one_shot}
\end{table}

==> Table/Other_methods.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
                         & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Text\\ Alignment\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Image\\ Alignment\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Subject\\ Alignment\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Background\\ Alignment\end{tabular}} \\
\midrule                 
Dreambooth               & 0.308                                                                        & \textbf{0.795}                                                                & 0.710                                                                           & 0.702                                                                              \\
Dreambooth + Ours        & \textbf{0.316}                                                               & 0.773                                                                         & \textbf{0.721}                                                                  & \textbf{0.683}                                                                     \\
\midrule
Custom Diffusion         & 0.293                                                                        & \textbf{0.815}                                                                & \textbf{0.732}                                                                  & 0.722                                                                              \\
Custom Diffusion + Ours  & \textbf{0.312}                                                               & 0.781                                                                         & 0.729                                                                           & \textbf{0.692}                                                                     \\
\midrule
SVDiff                   & 0.319                                                                        & \textbf{0.767}                                                                & 0.701                                                                           & 0.692                                                                              \\
SVDiff + Ours            & \textbf{0.324}                                                               & 0.745                                                                         & \textbf{0.704}                                                                  & \textbf{0.673}                                                                     \\
\midrule
Textual Inversion        & \textbf{0.292}                                                               & \textbf{0.762}                                                                & 0.707                                                                           & 0.694                                                                              \\
Textual Inversion + Ours & 0.289                                                                        & 0.753                                                                         & \textbf{0.719}                                                                  & \textbf{0.684}                                                                    \\
\bottomrule
\end{tabular}%
}
\caption{Compatibility on other methods.}
\label{tab:other_methods}
\end{table}

==> Table/Prompt_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
                                                Prompt design      & \begin{tabular}[c]{@{}c@{}}Text\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Image\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Subject\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Background\\ Alignment\end{tabular} \\
\midrule
Baseline                                              & 0.290                                                    & \textbf{0.781}                                            & 0.686                                                       & 0.701                                                          \\
Undesirable contents identification                      & 0.311                                                    & 0.729                                                     & \textbf{0.688}                                              & 0.658                                                          \\
Undesirable contents description & 0.317                                                    & 0.718                                                     & 0.681                                                       & \textbf{0.651}                                                 \\
Single content description & 0.312                                                    & 0.730                                                     & 0.687                                                       & 0.660                                                 \\
Subject desctiption                                   & \textbf{0.325}                                           & 0.696                                                     & 0.659                                                       & 0.652                                                          \\
Wrong description                                     & 0.303                                                    & 0.748                                                     & 0.688                                                       & 0.677                                                         \\
\bottomrule
\end{tabular}%
}
\caption{Quantitative evaluation on prompt design.}
\label{tab:prompt_ablation}
\end{table}

==> Table/Prompt_generator.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\begin{tabular}[c]{@{}l@{}}Prompt \\ Generator\end{tabular} & \begin{tabular}[c]{@{}c@{}}Text\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Image\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Subject\\ Alignment\end{tabular} & \begin{tabular}[c]{@{}c@{}}Background\\ Alignment\end{tabular} \\
\midrule
Baseline                                                    & 0.308                                                    & \textbf{0.795}                                            & 0.710                                                       & 0.702                                                          \\
GPT4                                                        & 0.316                                                    & 0.773                                                     & \textbf{0.721}                                              & 0.683                                                          \\
LLaVA                                                       & \textbf{0.319}                                           & 0.762                                                     & 0.713                                                       & \textbf{0.681}                                                 \\
BLIP2                                                       & 0.314                                                    & 0.780                                                     & 0.719                                                       & 0.691                                                          \\
Human                                                       & 0.315                                                    & 0.777                                                     & 0.721                                                       & 0.688                                                         \\
\bottomrule
\end{tabular}%
}
\caption{Ablation study on prompt generator.}
\label{tab:prompt_generator}
\end{table}
